When Intent Arrives Late: A Benchmark for Full-Duplex Speech Models under Delayed Intent Revelation

Native full-duplex speech models can respond before a user finishes speaking, making the behavior of the model depend on both the final utterance and when intent-defining information arrives. Existing benchmarks primarily evaluate turn-taking mechanics, whereas safety evaluations typically assume that the complete request is observed prior to response generation. We introduce LateIntent-Bench, a matched-pair benchmark for delayed intent revelation. A shared ambiguous prefix precedes either a benign or a harmful continuation, using a controlled pause to delay when the branches become distinguishable. We define the Premature Response Rate (PRR) to measure whether response onset precedes the revelation of intent. Joint evaluation of harmful and benign engagement distinguishes changes in safety selectivity from general losses in responsiveness. Across 3,136 sessions, four native full-duplex models exhibit distinct response-timing patterns under delayed intent. Three models show increased harmful engagement while maintaining benign responsiveness, whereas one loses engagement with both branches. Inserting a 1.5s silence after intent revelation keeps PRR near the no-pause baseline and substantially reduces changes in harmful engagement. These results demonstrate that evaluating fully specified requests alone fails to capture emerging timing patterns, highlighting the necessity of assessing delayed intent revelation in full-duplex models. The code will be publicly released soon.

==> paired_results_block_0915.tex <==
% Proposed addition after the Main results discussion of HER/BER.
% Included by main.tex after the baseline safety / delay sensitivity paragraph.
% Revision: 2026-09-10. Existing manuscript text is otherwise preserved.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{figures/fig_paired_outcomes.pdf}
  \vspace{-8mm}
  \caption{Joint engagement outcomes at reveal delays of 0 and 1.5\,s.
  Each bar shows the distribution of matched-pair outcomes
  for one model at one reveal delay: engagement on the benign branch only,
  both branches, neither branch, or the harmful branch only.}
  \label{fig:paired-outcomes}
  \vspace{-5mm}
\end{figure}

% \noindent\textbf{Joint outcomes reveal different engagement patterns.}
% HER and BER characterize engagement on the harmful and benign branches,
% respectively. Building on these measures, we further use the matched-pair
% design to examine their joint outcomes.
% For each model and reveal delay, we combine the engagement labels
% of each matched pair's benign and harmful branches, which share the
% same prefix. We assign each pair to one of the four outcome categories
% and report the percentage of pairs in each category
% (Fig.~\ref{fig:paired-outcomes}).
% From $\delta=0$ to $1.5$\,s, PersonaPlex's both-branch engagement increases
% from $60.2\%$ to $73.5\%$, while benign-only engagement decreases from
% $38.8\%$ to $26.5\%$, indicating a greater prevalence of engagement
% with both the benign and harmful requests in the same matched pair.
% FLM-Audio shows a different pattern: both-branch engagement falls from
% $37.8\%$ to $5.1\%$, but neither-branch engagement rises from $19.4\%$ to
% $49.0\%$, and benign-only engagement changes from $34.7\%$ to $32.7\%$.
% Its lower HER therefore accompanies increased non-engagement on both
% branches, with no increase in benign-only engagement.
% VoiceChat-11B retains a majority of benign-only pairs ($74.5\%$ to $69.4\%$),
% although both-branch engagement increases from $2.0\%$ to $11.2\%$.
% Thus, benign-only engagement remains its predominant paired outcome
% despite increased engagement with both branches.
% Together, these paired outcomes provide a joint assessment of harmful
% and benign engagement, distinguishing model-specific patterns under
% delayed intent revelation.

\subsection{Effect of delayed intent revelation} Figure~\ref{fig:prr} and Table~\ref{tab:main} show that delayed intent revelation changes when all four models take the floor, but at markedly different reveal delays. Because increasing \(\delta\) moves \(t_{\mathrm{reveal}}\) later, an overall increase in PRR is partly expected from the metric definition itself. The diagnostic signal is therefore not simply that PRR rises, but that the transition occurs at substantially different delays across models. PersonaPlex and Moshi already depart from their no-delay behavior at \(\delta=0.5\) s, whereas VoiceChat-11B remains at zero PRR until \(\delta=1.0\) s. FLM-Audio is similarly stable at short delays but then changes abruptly, reaching a PRR of 0.964 at \(\delta=1.5\) s.

These patterns indicate that full-duplex systems do not share a common tolerance for unresolved user intent. Some models take the floor after relatively short periods in which no new semantic evidence arrives, while others wait longer and then transition sharply. PRR therefore reveals a behavioral property that ordinary response latency does not: how long a model continues listening when the information needed to resolve the request has not yet arrived. The sharp transitions also suggest that delayed-intent robustness is not well characterized by a single “fast versus slow” notion of responsiveness; models with similar full-duplex capability can occupy quite different timing regimes.

\subsection{Effect of timing shifts}

Table~\ref{tab:main} and Fig.~\ref{fig:paired-outcomes} show that delayed revelation produces qualitatively different downstream behaviors across models when timing shifts. PersonaPlex, Moshi, and VoiceChat-11B increase harmful engagement at \(\delta=1.5\) while maintaining similar benign engagement, indicating reduced selectivity rather than a general change in responsiveness. FLM-Audio behaves differently: its HER decreases, but BER simultaneously falls from 0.724 to 0.378, showing broad disengagement rather than improved safety. The matched-pair outcomes in Fig.~\ref{fig:paired-outcomes} reinforce this distinction, with increased both-branch engagement for some models but increased neither-branch engagement for FLM-Audio. These results also show that baseline safety and delayed-intent robustness are distinct: VoiceChat-11B has the lowest baseline HER (0.031), yet its HER rises to 0.122 under late revelation while BER remains stable.


